Measurement-induced entanglement and teleportation on a noisy quantum processor

Measurement has a special role in quantum theory: by collapsing the wavefunction it can enable phenomena such as teleportation and thereby alter the "arrow of time" that constrains unitary evolution. When integrated in many-body dynamics, measurements can lead to emergent patterns of quantum information in space-time that go beyond established paradigms for characterizing phases, either in or out of equilibrium. On present-day NISQ processors, the experimental realization of this physics is challenging due to noise, hardware limitations, and the stochastic nature of quantum measurement. Here we address each of these experimental challenges and investigate measurement-induced quantum information phases on up to 70 superconducting qubits. By leveraging the interchangeability of space and time, we use a duality mapping, to avoid mid-circuit measurement and access different manifestations of the underlying phases -- from entanglement scaling to measurement-induced teleportation -- in a unified way. We obtain finite-size signatures of a phase transition with a decoding protocol that correlates the experimental measurement record with classical simulation data. The phases display sharply different sensitivity to noise, which we exploit to turn an inherent hardware limitation into a useful diagnostic. Our work demonstrates an approach to realize measurement-induced physics at scales that are at the limits of current NISQ processors.

==> packages.tex <==
\usepackage[T1]{fontenc}
%\usepackage[latin9]{inputenc}
%\usepackage[autopunct=true]{csquotes}
\usepackage{amsmath}
\usepackage{amssymb}
%\usepackage[intlimits]{amsmath}
\usepackage{amsmath}
%\usepackage{array}
\usepackage{graphicx}
\usepackage{esvect}
\usepackage{verbatim}
\usepackage{floatrow}
\usepackage{booktabs}
\usepackage{multirow}
%\usepackage{hyperref}
%\usepackage{scrextend}
\usepackage{blindtext}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{amssymb}
%\usepackage[hidelinks]{hyperref}
\usepackage[table]{xcolor}

% \usepackage[demo]{graphicx}
\usepackage{floatrow}
\makeatletter

% \usepackage[usenames,dvipsnames]{color}
%  \@ifundefined{textcolor}{}
%  {
%   \definecolor{BLACK}{gray}{0}
%   \definecolor{WHITE}{gray}{1}
%   \definecolor{RED}{rgb}{0.75,0,0}
%   \definecolor{GREEN}{rgb}{0.0,0.75,0.0}
%   \definecolor{BLUE}{rgb}{0,0,0.75}
%   \definecolor{CYAN}{cmyk}{1,0,0,0}
%   \definecolor{darkred}{cmyk}{0,1,0,0.45}
%   \definecolor{MAGENTA}{cmyk}{0,1,0,0}
%   \definecolor{YELLOW}{cmyk}{0,0,1,0}
%     \definecolor{SECTIONCOLOR}{rgb}{0,0,0.65}
%   \definecolor{SUBSECTIONCOLOR}{rgb}{0.0,0.0,0.75}
%   \definecolor{SUBSUBSECTIONCOLOR}{rgb}{0,0.6,0}
%  }
% \definecolor{light-gray}{gray}{0.55}

%\usepackage{babel}
\newcommand{\psection}[1]{\textcolor{BLUE}{\textbf{\emph{#1}}}}
\newcommand{\newln}{\\&\quad\quad{}}
\newcommand{\parenthnewln}{\right.\\&\left.\quad\quad{}}

\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

\renewcommand{\thefigure}{\arabic{figure}}
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}
\renewcommand*\l@subsection{\@dottedtocline{2}{1.8em}{3.2 em}}
\renewcommand*\l@subsubsection{\@dottedtocline{2}{1.8em}{6.4 em}}

\setlength{\belowcaptionskip}{0pt}
\addtolength{\columnsep}{-0pt}
\addtolength{\textwidth}{0pt}

\g@addto@macro\normalsize{%
  \setlength\abovedisplayskip{0pt}
  \setlength\belowdisplayskip{0pt}
  \setlength\abovedisplayshortskip{0pt}
 \setlength\belowdisplayshortskip{0pt}
}

\newcommand{\numberofqubits}{n}
\newcommand{\schrodinger}{Schr\"{o}dinger}
\newcommand{\xebfidelity}{ \mathcal{F}_{\text{XEB}} }
